Lifted Disjoint Paths with Application in Multiple Object Tracking

We present an extension to the disjoint paths problem in which additional \emph{lifted} edges are introduced to provide path connectivity priors. We call the resulting optimization problem the lifted disjoint paths problem. We show that this problem is NP-hard by reduction from integer multicommodity flow and 3-SAT. To enable practical global optimization, we propose several classes of linear inequalities that produce a high-quality LP-relaxation. Additionally, we propose efficient cutting plane algorithms for separating the proposed linear inequalities. The lifted disjoint path problem is a natural model for multiple object tracking and allows an elegant mathematical formulation for long range temporal interactions. Lifted edges help to prevent id switches and to re-identify persons. Our lifted disjoint paths tracker achieves nearly optimal assignments with respect to input detections. As a consequence, it leads on all three main benchmarks of the MOT challenge, improving significantly over state-of-the-art.

==> mot15_result.tex <==
 Method & AvgRank$\downarrow$ & MOTA$\uparrow$  & IDF1$\uparrow$  & MT$\uparrow$  & ML$\downarrow$  & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ & Frag$\downarrow$ \\  
 LNF\_15 & \textbf{18.8} & \textbf{52.5} & \textbf{60} & \textbf{33.8}  & \textbf{25.8} & 6837 & \textbf{21610} & 730 & \textbf{1047}  \\ 
 Tracktor15 \cite{bergmann2019tracking} & 35.3 & 44.1 & 46.7 & 18.0 & 26.2 & 6477 & 26577 & 1318 & 1790  \\ 
 KCF \cite{chu2019online} & 30.4 & 38.9 & 44.5 & 16.6 & 31.5 & 7321 & 29501 & 720 & 1440  \\ 
 AP\_HWDPL\_p \cite{chen2017online} & 22.6 & 38.5 & 47.1 & 8.7 & 37.4  & \textbf{4005} & 33203 & \textbf{586} & 1263  \\ 
 STRN \cite{xu2019spatial} & 33.7 & 38.1 & 46.6 & 11.5 & 33.4  & 5451 & 31571 & 1033 & 2665  \\ 
 AMIR15 \cite{sadeghian2017tracking} & 30.8 & 37.6 & 46 & 15.8 & 26.8 & 7933 & 29397 & 1026 & 2024   

==> mot16_result.tex <==
 Method & AvgRank$\downarrow$ & MOTA$\uparrow$  & IDF1$\uparrow$  & MT$\uparrow$  & ML$\downarrow$  & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ & Frag$\downarrow$ \\    
 LNF & \textbf{20.3} & \textbf{61.3} & \textbf{64.7} & \textbf{27.0} & \textbf{34.0} & 4844 & \textbf{65401} & \textbf{389} & 1034  \\ 
 Tracktor\cite{bergmann2019tracking}\footnote{\label{foot:TracktorDPM} The tracker uses a different input set of DPM detections (without the non-maxima-surpression)}  & 41.4 & 54.4 & 52.5 & 19.0 & 36.9 & \textbf{3280} & 79149 & 682 & 1480  \\ 
 NOTA \cite{chen2019aggregate} & 38.7 & 49.8 & 55.3 & 17.9 & 37.7 & 7248 & 83614 & 614 & 1372  \\ 
 HCC \cite{ma2018customized} & 38.3 & 49.3 & 50.7 & 17.8 & 39.9 & 5333 & 86795 & 391 & \textbf{535}  \\ 
 eTC \cite{wang2019exploit} & 42.5 & 49.2 & 56.1 & 17.3 & 40.3 & 8400 & 83702 & 606 & 882  \\ 
 KCF16 \cite{chu2019online} & 56.3 & 48.8 & 47.2 & 15.8 & 38.1 & 5875 & 86567 & 906 & 1116  

==> mot17_result.tex <==
 Method & AvgRank$\downarrow$ & MOTA$\uparrow$  & IDF1$\uparrow$  & MT$\uparrow$  & ML$\downarrow$  & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ & Frag$\downarrow$ \\   
 LDP & \textbf{24.8} & \textbf{60.5} & \textbf{65.6} & \textbf{27.0}  & 33.6  & 14966 & \textbf{206619} & \textbf{1189} & 3476  \\ 
 Tracktor17 \cite{bergmann2019tracking}\footnoteref{foot:TracktorDPM} & 54.8 & 53.5 & 52.3 & 19.5 & 36.6  & \textbf{12201} & 248047 & 2072 & 4611  \\ 
 JBNOT \cite{henschel2019multiple}  & 55 & 52.6 & 50.8 & 19.7 & 35.8 & 31572 & 232659 & 3050 & 3792  \\ 
 FAMNet \cite{chu2019famnet} & 58.4 & 52 & 48.7 & 19.1 & \textbf{33.4}  & 14138 & 253616 & 3072 & 5318  \\ 
 eTC17 \cite{wang2019exploit} & 45.4 & 51.9 & 58.1 & 23.1  & 35.5  & 36164 & 232783 & 2288 & 3071  \\ 
 eHAF17 \cite{sheng2018heterogeneous} & 46.9 & 51.8 & 54.7 & 23.4  & 37.9  & 33212 & 236772 & 1834 & \textbf{2739}   
